Structure determinations for random-tiling quasicrystals

How, in principle, could one solve the atomic structure of a quasicrystal, modeled as a random tiling decorated by atoms, and what techniques are available to do it? One path is to solve the phase problem first, obtaining the density in a higher dimensional space which yields the_averaged_ scattering density in 3-dimensional space by the usual construction of an incommensurate cut. A novel direct method for this is summarized and applied to an i(AlPdMn) data set. This averaged density falls short of a true structure determination (which would reveal the typical_unaveraged_ atomic patterns.) We discuss the problematic validity of inferring an ideal structure by simply factoring out a ``perp-space'' Debye-Waller factor, and we test this using simulations of rhombohedral tilings. A second, ``unified'' path is to relate the measured and modeled intensities directly, by adjusting parameters in a simulation to optimize the fit. This approach is well suited for unifying structural information from diffraction and from minimizing total energies derived ultimately from ab-initio calculations. Finally, we discuss the special pitfalls of fitting random-tiling decagonal phases.

==> elements.tex <==
%auto-ignore

%Zeitschrift fuer Kristallographie, Oldenbourg Muenchen

\renewcommand{\Title}
{Structure determinations for random-tiling quasicrystals}

                   % Footnotenumbers (strongly discommended) in Title 
                   % have to be constructed. Do not use the footnote command. 
                   % It might be necessary to typeset the footnotenumber in italics 
                   % to distinguish from chemical formulae (e.g. H$_2$O$^{\mathit 1}$)
                   % The usual footnotetext must be placed at a suitable spot later on. 
                   % The belonging footnote should appear with the standard (upright) number

\renewcommand{\AuthorsComplete}
{C.~L.~Henley$^*$, V.~Elser, and M.~Mihalkovi\v{c}\protect\footnote
{MM address}}

                   % with all additions (e.g. constructed footnotemarks)
                   % the one footnotemark for the corresponding author (one only, please!) 
                   % is mandatory, the appropriate footnotetext appears automatically

\renewcommand{\CorrespondenceAuthor}{(e-mail: clh@ccmr.cornell.edu)
Please also note that M.M.'s 
present address is
Materials Research and Liquids, Institute of Physics,
TU Chemnitz, D-09107 Chemnitz, Germany;
his permanent address,
Institute of Physics, Slovak Academy of Sciences, 84228 Bratislava, Slovakia.
}
                   % absolutely preferred: (email) only

\renewcommand{\InstitutionOne}
{LASSP, Cornell University, Ithaca NY 14853-2501.}
          %will appear under I ifmore than one 
\renewcommand{\InstitutionTwo}{}     %will appear under II
\renewcommand{\InstitutionThree}{}   %will appear under III 
\renewcommand{\InstitutionFour}{}    %will appear under IV 
\renewcommand{\InstitutionFive}{}    %will appear under V 
\renewcommand{\InstitutionSix}{}     %will appear under VI 


%%% Marek's
%%% Current address:
%%% Materials Research and Liquids, Institute of Physics,
%%% TU Chemnitz, D-09107 Chemnitz, Germany;
%%% permanent address, Institute of Physics, 
%%% Slovak Academy of Sciences, 84228 Bratislava, Slovakia.


\renewcommand{\SayThanks}{}

\renewcommand{\Abstract}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{How, in principle,  could one solve the atomic
structure of a quasicrystal, modeled as a random tiling decorated
by atoms, and what techniques are available to do it?
One path is to solve the phase problem first, obtaining
the density in a higher dimensional space which yields 
the {\it averaged} scattering density in 3-dimensional space
by the usual construction of an incommensurate cut.
A novel direct method for this is summarized and applied to 
an $i$(AlPdMn) data set.
This averaged density falls short of a true structure determination
(which would reveal the typical {\it unaveraged} atomic patterns.)
We discuss the problematic validity of inferring an ideal structure 
by simply factoring out a ``perp-space'' Debye-Waller factor, and
we test this using simulations of rhombohedral tilings.
A second, ``unified'' path is to relate the measured and modeled
intensities directly, by adjusting parameters in a simulation to optimize
the fit.  This approach is well suited for 
unifying structural information from diffraction and from
minimizing total energies derived ultimately from ab-initio
calculations. Finally, we discuss the special pitfalls of
fitting random-tiling decagonal phases.}


%%%%%%%%%%%%%%%%%%%%%%% for publisher only %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\Paperreceived}{} % date only; format: April 23, 1998
\renewcommand{\Paperaccepted}{}  % date only; format: April 24, 1998
\setcounter{Papervolume}{216}                 %publisher: volume number here
%\setcounter{page}{}                          % publisher: pagenumber here

\renewcommand{\Authors}{} % without any additions for databank purposes

\renewcommand{\cleanTitle}{}   % only needed to eliminate additions from Title 
                               % like footnotes etc. for databank purposes
\renewcommand{\shortAuthors}{} % only needed for headings; else = Authors
\renewcommand{\shortTitle}{Structure determinations for
random-tiling quasicrystals}   % only needed for headings; else = cleanTitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput



